Towards Clear Expectations for Uncertainty Estimation

If Uncertainty Quantification (UQ) is crucial to achieve trustworthy Machine Learning (ML), most UQ methods suffer from disparate and inconsistent evaluation protocols. We claim this inconsistency results from the unclear requirements the community expects from UQ. This opinion paper offers a new perspective by specifying those requirements through five downstream tasks where we expect uncertainty scores to have substantial predictive power. We design these downstream tasks carefully to reflect real-life usage of ML models. On an example benchmark of 7 classification datasets, we did not observe statistical superiority of state-of-the-art intrinsic UQ methods against simple baselines. We believe that our findings question the very rationale of why we quantify uncertainty and call for a standardized protocol for UQ evaluation based on metrics proven to be relevant for the ML practitioner.

==> tables/agnostic_binary.tex <==
\begin{tabular}{llllllll}
\toprule

                          Model &           Score &                                             Retention &                                       Error Detection &                OoD Detection &             OoD Detection (AUC) &                           Shift Detection &                                  Performance Drop Prediction \\
\toprule
\midrule 
                       Black-Box &  max confidence &  \textbf{0.948}
                       $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.790} $|$ \underline{1.0} / \underline{1.0} &          -0.008 $|$ 0.2 / 0.4 &           0.503 $|$ 0.2 / 0.6 &  \textbf{0.738} $|$ \underline{1.0} / 0.7 &  \textbf{0.100} $|$ \underline{1.0} / \underline{1.0} \\
\midrule
            Isotonic Calibration &  max confidence &              \textbf{0.948} $|$ \underline{1.0} / 0.9 &                                   0.782 $|$ 0.2 / 0.9 &  \textbf{0.014} $|$ 0.8 / 0.4 &           0.496 $|$ 0.0 / 0.4 &                       0.604 $|$ 0.2 / 0.4 &                                   0.111 $|$ 0.2 / 0.1 \\
\midrule
CP (confidence) &          pvalue &                                   0.943 $|$ 0.0 / 0.4 &                                   0.735 $|$ 0.0 / 0.3 &          -0.040 $|$ 0.0 / 0.4 &  \textbf{0.508} $|$ 0.8 / 0.4 &                       0.595 $|$ 0.0 / 0.3 &                                   0.105 $|$ 1.0 / 0.6 \\
 &     credibility &                                   0.937 $|$ 0.0 / 0.4 &                                   0.695 $|$ 0.0 / 0.3 &          -0.079 $|$ 0.0 / 0.4 &           0.505 $|$ 0.2 / 0.4 &                       0.538 $|$ 0.0 / 0.3 &                                   0.113 $|$ 0.2 / 0.4 \\
  &      confidence &                                   0.937 $|$ 0.0 / 0.3 &                                   0.692 $|$ 0.0 / 0.3 &          -0.100 $|$ 0.0 / 0.0 &           0.497 $|$ 0.0 / 0.1 &                       0.480 $|$ 0.0 / 0.3 &                                   0.111 $|$ 0.5 / 0.6 \\
 &      efficiency &                                   0.932 $|$ 0.0 / 0.0 &                                   0.657 $|$ 0.0 / 0.0 &          -0.067 $|$ 0.0 / 0.4 &           0.499 $|$ 0.2 / 0.3 &                       0.377 $|$ 0.0 / 0.1 &                                   0.219 $|$ 0.0 / 0.1 \\
\bottomrule
\toprule
\end{tabular}

==> tables/agnostic_multiclass.tex <==
\begin{tabular}{lllllll}
\toprule
                           Model &           Score &                                 Retention &                           Error detection &                            OoD Detection &                           Shift Detection &                     Performance Drop Prediction \\
\midrule

Black-Box &  max confidence &  \textbf{0.880} $|$ 0.8 / \underline{1.0} &  \textbf{0.786} $|$ 0.8 / \underline{1.0} &                      -0.009 $|$ 0.5 / 0.5 &                       0.974 $|$ 0.8 / 0.8 &              \textbf{0.143} $|$ 0.8 / 0.5 \\
 &          margin &              \textbf{0.879} $|$ 0.5 / 0.8 &                       0.781 $|$ 0.0 / 0.2 &  \textbf{0.040} $|$ \underline{1.0} / 0.5 &                       0.962 $|$ 0.5 / 0.5 &  \textbf{0.132} $|$ \underline{1.0} / 0.5 \\
&         entropy &              \textbf{0.879} $|$ 0.5 / 0.5 &                       0.775 $|$ 0.0 / 0.2 &                      -0.058 $|$ 0.2 / 0.2 &  \textbf{0.991} $|$ \underline{1.0} / 0.8 &                       0.170 $|$ 0.8 / 0.2 \\
\midrule
Isotonic Calibration &  max confidence &                       0.878 $|$ 0.5 / 0.5 &                       0.772 $|$ 0.5 / 0.5 &                       0.016 $|$ 0.8 / 0.2 &                       0.945 $|$ 0.5 / 0.8 &  \textbf{0.134} $|$ \underline{1.0} / 0.8 \\
 &          margin &                       0.875 $|$ 0.2 / 0.2 &                       0.761 $|$ 0.2 / 0.0 &              \textbf{0.066} $|$ 0.8 / 0.5 &                       0.943 $|$ 0.5 / 0.8 &  \textbf{0.131} $|$ \underline{1.0} / 0.5 \\
 &         entropy &                       0.876 $|$ 0.0 / 0.2 &                       0.763 $|$ 0.0 / 0.0 &                      -0.039 $|$ 0.2 / 0.2 &                       0.952 $|$ 0.5 / 0.8 &              \textbf{0.143} $|$ 0.8 / 0.2 \\
 \midrule
CP (confidence) &      confidence &                       0.868 $|$ 0.0 / 0.0 &                       0.722 $|$ 0.0 / 0.0 &                       0.002 $|$ 0.2 / 0.2 &                       0.893 $|$ 0.2 / 0.2 &                       0.184 $|$ 0.0 / 0.0 \\
&          pvalue &                       0.866 $|$ 0.0 / 0.0 &                       0.690 $|$ 0.0 / 0.0 &                      -0.019 $|$ 0.5 / 0.2 &                       0.831 $|$ 0.2 / 0.8 &                       0.153 $|$ 0.8 / 0.2 \\
 &     credibility &                       0.859 $|$ 0.0 / 0.0 &                       0.662 $|$ 0.0 / 0.0 &                      -0.054 $|$ 0.5 / 0.2 &                       0.812 $|$ 0.2 / 0.8 &                       0.159 $|$ 0.8 / 0.2 \\
  &      efficiency &                       0.863 $|$ 0.0 / 0.0 &                       0.673 $|$ 0.0 / 0.0 &                      -0.116 $|$ 0.0 / 0.2 &                       0.758 $|$ 0.0 / 0.0 &                       0.253 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}

==> tables/conformal_binary.tex <==
\begin{tabular}{llllllll}
\toprule
                           model &           score &                                 retention &                                       error detection &                             ood detection &                         ood detection auc &                           shift detection &                      perf drop prediction \\
\toprule
CP (Confidence) &  non-conformity &  \textbf{0.948} $|$ \underline{1.0} / 0.9 &  \textbf{0.790} $|$ \underline{1.0} / \underline{1.0} &                      -0.008 $|$ 0.0 / 0.0 &                       0.503 $|$ 0.0 / 0.3 &                       0.739 $|$ 0.0 / 0.1 &  \textbf{0.100} $|$ \underline{1.0} / 0.7 \\
&          pvalue &                       0.943 $|$ 0.0 / 0.3 &                                   0.735 $|$ 0.0 / 0.3 &                      -0.040 $|$ 0.0 / 0.0 &                       0.508 $|$ 0.0 / 0.0 &                       0.598 $|$ 0.0 / 0.1 &                       0.105 $|$ 0.8 / 0.6 \\
 &     credibility &                       0.937 $|$ 0.0 / 0.3 &                                   0.695 $|$ 0.0 / 0.3 &                      -0.079 $|$ 0.0 / 0.0 &                       0.505 $|$ 0.0 / 0.0 &                       0.545 $|$ 0.0 / 0.0 &                       0.113 $|$ 0.2 / 0.4 \\
 &      confidence &                       0.937 $|$ 0.0 / 0.1 &                                   0.692 $|$ 0.0 / 0.3 &                      -0.100 $|$ 0.0 / 0.0 &                       0.497 $|$ 0.0 / 0.0 &                       0.479 $|$ 0.0 / 0.0 &                       0.111 $|$ 0.2 / 0.4 \\
 &      efficiency &                       0.932 $|$ 0.0 / 0.0 &                                   0.657 $|$ 0.0 / 0.0 &                      -0.067 $|$ 0.0 / 0.0 &                       0.499 $|$ 0.0 / 0.0 &                       0.372 $|$ 0.0 / 0.0 &                       0.219 $|$ 0.0 / 0.0 \\
  \midrule 
CP (Trust score) &  non-conformity &                       0.937 $|$ 0.0 / 0.3 &                                   0.710 $|$ 0.0 / 0.1 &                       0.192 $|$ 0.0 / 0.0 &                       0.544 $|$ 0.0 / 0.1 &                       0.798 $|$ 0.0 / 0.1 &              \textbf{0.102} $|$ 0.8 / 0.3 \\
 &          pvalue &                       0.934 $|$ 0.0 / 0.3 &                                   0.678 $|$ 0.0 / 0.1 &                       0.157 $|$ 0.0 / 0.0 &                       0.549 $|$ 0.0 / 0.0 &                       0.701 $|$ 0.0 / 0.1 &                       0.116 $|$ 0.2 / 0.1 \\
 &     credibility &                       0.921 $|$ 0.0 / 0.1 &                                   0.596 $|$ 0.0 / 0.0 &                       0.128 $|$ 0.0 / 0.0 &                       0.568 $|$ 0.0 / 0.0 &                       0.659 $|$ 0.0 / 0.0 &                       0.137 $|$ 0.0 / 0.1 \\
 
&      confidence &                       0.921 $|$ 0.0 / 0.0 &                                   0.586 $|$ 0.0 / 0.0 &                       0.105 $|$ 0.0 / 0.0 &                       0.575 $|$ 0.0 / 0.0 &                       0.544 $|$ 0.0 / 0.0 &                       0.143 $|$ 0.0 / 0.0 \\
 &      efficiency &                       0.919 $|$ 0.0 / 0.0 &                                   0.574 $|$ 0.0 / 0.0 &                       0.032 $|$ 0.0 / 0.0 &                       0.539 $|$ 0.0 / 0.0 &                       0.297 $|$ 0.0 / 0.0 &                       0.219 $|$ 0.0 / 0.0 \\
\midrule
CP (Anomaly score) &  non conformity &                       0.922 $|$ 0.0 / 0.0 &                                   0.626 $|$ 0.0 / 0.0 &  \textbf{0.798} $|$ \underline{1.0} / 0.7 &                       0.638 $|$ 0.8 / 0.4 &  \textbf{0.915} $|$ \underline{1.0} / 0.6 &                       0.178 $|$ 0.0 / 0.4 \\

 &          pvalue &                       0.920 $|$ 0.0 / 0.0 &                                   0.604 $|$ 0.0 / 0.0 &                       0.777 $|$ 0.2 / 0.1 &  \textbf{0.641} $|$ \underline{1.0} / 0.6 &                       0.852 $|$ 0.0 / 0.3 &                       0.178 $|$ 0.0 / 0.6 \\
 &      confidence &                       0.919 $|$ 0.0 / 0.0 &                                   0.546 $|$ 0.0 / 0.0 &                      -0.814 $|$ 0.0 / 0.0 &                       0.415 $|$ 0.0 / 0.1 &                       0.864 $|$ 0.2 / 0.4 &                       0.154 $|$ 0.0 / 0.0 \\
 &     credibility &                       0.917 $|$ 0.0 / 0.0 &                                   0.573 $|$ 0.0 / 0.0 &                       0.789 $|$ 0.5 / 0.6 &              \textbf{0.640} $|$ 0.8 / 0.6 &                       0.849 $|$ 0.0 / 0.3 &                       0.180 $|$ 0.0 / 0.6 \\

 &      efficiency &                       0.918 $|$ 0.0 / 0.0 &                                   0.553 $|$ 0.0 / 0.0 &                       0.108 $|$ 0.0 / 0.0 &                       0.533 $|$ 0.0 / 0.0 &                       0.337 $|$ 0.0 / 0.0 &                       0.147 $|$ 0.0 / 0.1 \\
 \midrule
  CP (Hashing score)  &  non conformity &                       0.917 $|$ 0.0 / 0.0 &                                   0.494 $|$ 0.0 / 0.0 &                      -0.006 $|$ 0.0 / 0.0 &                       0.502 $|$ 0.0 / 0.0 &                       0.033 $|$ 0.0 / 0.0 &                       0.123 $|$ 0.0 / 0.4 \\
  
 &          pvalue &                       0.917 $|$ 0.0 / 0.0 &                                   0.494 $|$ 0.0 / 0.0 &                      -0.005 $|$ 0.0 / 0.0 &                       0.502 $|$ 0.0 / 0.0 &                       0.034 $|$ 0.0 / 0.0 &                       0.123 $|$ 0.0 / 0.4 \\
&      confidence &                       0.917 $|$ 0.0 / 0.0 &                                   0.509 $|$ 0.0 / 0.0 &                       0.004 $|$ 0.0 / 0.0 &                       0.500 $|$ 0.0 / 0.0 &                       0.017 $|$ 0.0 / 0.0 &                       0.125 $|$ 0.0 / 0.4 \\
 &      efficiency &                       0.917 $|$ 0.0 / 0.0 &                                   0.502 $|$ 0.0 / 0.0 &                       0.004 $|$ 0.0 / 0.0 &                       0.501 $|$ 0.0 / 0.0 &                       0.000 $|$ 0.0 / 0.0 &                       0.217 $|$ 0.0 / 0.1 \\
&     credibility &                       0.917 $|$ 0.0 / 0.0 &                                   0.497 $|$ 0.0 / 0.0 &                      -0.010 $|$ 0.0 / 0.0 &                       0.503 $|$ 0.0 / 0.0 &                       0.021 $|$ 0.0 / 0.0 &                       0.121 $|$ 0.0 / 0.4 \\

\bottomrule
\end{tabular}



==> tables/conformal_multiclass.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                             ood detection &                           shift detection &          perf drop prediction \\
\midrule
 confidence conformal prediction &  non conformity &  \textbf{0.880} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.786} $|$ \underline{1.0} / \underline{1.0} &                      -0.009 $|$ 0.0 / 0.0 &                       0.976 $|$ 0.0 / 0.0 &  \textbf{0.143} $|$ 0.5 / 0.2 \\
 confidence conformal prediction &      confidence &                                   0.868 $|$ 0.0 / 0.0 &                                   0.722 $|$ 0.0 / 0.0 &                       0.002 $|$ 0.0 / 0.0 &                       0.888 $|$ 0.0 / 0.0 &           0.184 $|$ 0.0 / 0.0 \\
      trust conformal prediction &  non conformity &                                   0.866 $|$ 0.0 / 0.2 &                                   0.721 $|$ 0.0 / 0.0 &                       0.081 $|$ 0.0 / 0.0 &                       0.997 $|$ 0.0 / 0.2 &           0.176 $|$ 0.0 / 0.0 \\
 confidence conformal prediction &          pvalue &                                   0.866 $|$ 0.0 / 0.0 &                                   0.690 $|$ 0.0 / 0.0 &                      -0.019 $|$ 0.0 / 0.0 &                       0.818 $|$ 0.0 / 0.0 &           0.153 $|$ 0.2 / 0.0 \\
 confidence conformal prediction &      efficiency &                                   0.863 $|$ 0.0 / 0.0 &                                   0.673 $|$ 0.0 / 0.0 &                      -0.116 $|$ 0.0 / 0.0 &                       0.755 $|$ 0.0 / 0.0 &           0.253 $|$ 0.0 / 0.0 \\
      trust conformal prediction &          pvalue &                                   0.860 $|$ 0.0 / 0.0 &                                   0.668 $|$ 0.0 / 0.0 &                       0.075 $|$ 0.0 / 0.0 &                       0.901 $|$ 0.0 / 0.0 &           0.164 $|$ 0.2 / 0.0 \\
 confidence conformal prediction &     credibility &                                   0.859 $|$ 0.0 / 0.0 &                                   0.662 $|$ 0.0 / 0.0 &                      -0.054 $|$ 0.0 / 0.0 &                       0.801 $|$ 0.0 / 0.0 &           0.159 $|$ 0.2 / 0.0 \\
    anomaly conformal prediction &      confidence &                                   0.850 $|$ 0.0 / 0.0 &                                   0.575 $|$ 0.0 / 0.0 &                      -0.683 $|$ 0.0 / 0.0 &  \textbf{1.000} $|$ \underline{1.0} / 0.0 &           0.244 $|$ 0.0 / 0.0 \\
      trust conformal prediction &     credibility &                                   0.844 $|$ 0.0 / 0.0 &                                   0.566 $|$ 0.0 / 0.0 &                      -0.056 $|$ 0.0 / 0.0 &                       0.904 $|$ 0.0 / 0.0 &           0.146 $|$ 0.2 / 0.0 \\
      trust conformal prediction &      confidence &                                   0.844 $|$ 0.0 / 0.0 &                                   0.598 $|$ 0.0 / 0.0 &                       0.276 $|$ 0.0 / 0.0 &              \textbf{1.000} $|$ 0.5 / 0.0 &           0.159 $|$ 0.2 / 0.0 \\
    anomaly conformal prediction &  non conformity &                                   0.843 $|$ 0.0 / 0.0 &                                   0.600 $|$ 0.0 / 0.0 &  \textbf{0.743} $|$ \underline{1.0} / 0.5 &  \textbf{1.000} $|$ \underline{1.0} / 0.0 &           0.217 $|$ 0.0 / 0.5 \\
    anomaly conformal prediction &      efficiency &                                   0.842 $|$ 0.0 / 0.0 &                                   0.550 $|$ 0.0 / 0.0 &                      -0.081 $|$ 0.0 / 0.0 &                       0.914 $|$ 0.0 / 0.0 &           0.306 $|$ 0.0 / 0.2 \\
      trust conformal prediction &      efficiency &                                   0.842 $|$ 0.0 / 0.0 &                                   0.586 $|$ 0.0 / 0.0 &                       0.148 $|$ 0.0 / 0.0 &                       0.681 $|$ 0.0 / 0.0 &           0.372 $|$ 0.0 / 0.0 \\
    anomaly conformal prediction &          pvalue &                                   0.841 $|$ 0.0 / 0.0 &                                   0.567 $|$ 0.0 / 0.0 &                       0.662 $|$ 0.0 / 0.0 &                       0.780 $|$ 0.0 / 0.0 &           0.214 $|$ 0.0 / 0.2 \\
    hashing conformal prediction &     credibility &                                   0.838 $|$ 0.0 / 0.0 &                                   0.504 $|$ 0.0 / 0.0 &                      -0.004 $|$ 0.0 / 0.0 &                       0.016 $|$ 0.0 / 0.0 &  \textbf{0.129} $|$ 0.8 / 0.2 \\
    hashing conformal prediction &  non conformity &                                   0.838 $|$ 0.0 / 0.0 &                                   0.499 $|$ 0.0 / 0.0 &                      -0.001 $|$ 0.0 / 0.0 &                       0.025 $|$ 0.0 / 0.0 &  \textbf{0.130} $|$ 0.8 / 0.2 \\
    hashing conformal prediction &          pvalue &                                   0.838 $|$ 0.0 / 0.0 &                                   0.500 $|$ 0.0 / 0.0 &                      -0.000 $|$ 0.0 / 0.0 &                       0.021 $|$ 0.0 / 0.0 &  \textbf{0.130} $|$ 0.8 / 0.2 \\
    hashing conformal prediction &      efficiency &                                   0.838 $|$ 0.0 / 0.0 &                                   0.497 $|$ 0.0 / 0.0 &                       0.001 $|$ 0.0 / 0.0 &                       0.000 $|$ 0.0 / 0.0 &           0.327 $|$ 0.0 / 0.0 \\
    hashing conformal prediction &      confidence &                                   0.837 $|$ 0.0 / 0.0 &                                   0.497 $|$ 0.0 / 0.0 &                       0.005 $|$ 0.0 / 0.0 &                       0.012 $|$ 0.0 / 0.0 &  \textbf{0.130} $|$ 0.8 / 0.2 \\
    anomaly conformal prediction &     credibility &                                   0.834 $|$ 0.0 / 0.0 &                                   0.528 $|$ 0.0 / 0.0 &                       0.719 $|$ 0.2 / 0.2 &                       0.772 $|$ 0.0 / 0.0 &           0.169 $|$ 0.2 / 0.2 \\
\bottomrule
\end{tabular}

==> tables/intrinsic_binary.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                             ood detection &                           shift detection &                      perf drop prediction \\
\midrule
                       intrinsic &           total &  \textbf{0.956} $|$ \underline{1.0} / \underline{1.0} &              \textbf{0.802} $|$ \underline{1.0} / 0.9 &                      -0.027 $|$ 0.0 / 0.0 &                       0.761 $|$ 0.5 / 0.4 &  \textbf{0.051} $|$ \underline{1.0} / 0.7 \\
 confidence conformal prediction &  non conformity &  \textbf{0.956} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.802} $|$ \underline{1.0} / \underline{1.0} &                      -0.033 $|$ 0.0 / 0.0 &                       0.756 $|$ 0.5 / 0.4 &  \textbf{0.050} $|$ \underline{1.0} / 0.7 \\
                       intrinsic &       aleatoric &  \textbf{0.956} $|$ \underline{1.0} / \underline{1.0} &              \textbf{0.801} $|$ \underline{1.0} / 0.7 &                      -0.075 $|$ 0.0 / 0.0 &                       0.757 $|$ 0.5 / 0.4 &                       0.069 $|$ 0.5 / 0.4 \\
            isotonic calibration &  max confidence &              \textbf{0.956} $|$ \underline{1.0} / 0.9 &                                   0.794 $|$ 0.0 / 0.7 &                      -0.010 $|$ 0.0 / 0.0 &                       0.595 $|$ 0.0 / 0.0 &                       0.068 $|$ 1.0 / 0.1 \\
 confidence conformal prediction &          pvalue &                                   0.949 $|$ 0.0 / 0.1 &                                   0.732 $|$ 0.0 / 0.1 &                      -0.078 $|$ 0.0 / 0.1 &                       0.498 $|$ 0.0 / 0.0 &  \textbf{0.051} $|$ \underline{1.0} / 0.7 \\
 confidence conformal prediction &      confidence &                                   0.945 $|$ 0.0 / 0.1 &                                   0.702 $|$ 0.0 / 0.1 &                      -0.130 $|$ 0.0 / 0.0 &                       0.476 $|$ 0.0 / 0.0 &  \textbf{0.057} $|$ \underline{1.0} / 0.7 \\
 confidence conformal prediction &     credibility &                                   0.945 $|$ 0.0 / 0.1 &                                   0.702 $|$ 0.0 / 0.1 &                      -0.104 $|$ 0.0 / 0.1 &                       0.481 $|$ 0.0 / 0.0 &  \textbf{0.055} $|$ \underline{1.0} / 0.6 \\
                       intrinsic &       epistemic &                                   0.943 $|$ 0.0 / 0.1 &                                   0.712 $|$ 0.0 / 0.1 &  \textbf{0.269} $|$ \underline{1.0} / 0.9 &  \textbf{0.802} $|$ \underline{1.0} / 0.6 &                       0.086 $|$ 0.0 / 0.6 \\
 confidence conformal prediction &      efficiency &                                   0.940 $|$ 0.0 / 0.0 &                                   0.665 $|$ 0.0 / 0.0 &                      -0.098 $|$ 0.0 / 0.0 &                       0.359 $|$ 0.0 / 0.0 &                       0.199 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}

==> tables/intrinsic_binary_catboost.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                             ood detection &                           shift detection &                      perf drop prediction \\
\toprule
Intrinsic &           total &              \textbf{0.957} $|$ \underline{1.0} / 0.9 &              \textbf{0.806} $|$ \underline{1.0} / 0.9 &                      -0.012 $|$ 0.0 / 0.1 &  \textbf{0.752} $|$ \underline{1.0} / 0.4 &  \textbf{0.042} $|$ \underline{1.0} / 0.9 \\
 &       aleatoric &              \textbf{0.957} $|$ \underline{1.0} / 0.9 &              \textbf{0.806} $|$ \underline{1.0} / 0.9 &                      -0.013 $|$ 0.0 / 0.1 &  \textbf{0.768} $|$ \underline{1.0} / 0.6 &  \textbf{0.042} $|$ \underline{1.0} / 0.9 \\
 &       epistemic &                                   0.939 $|$ 0.0 / 0.1 &                                   0.676 $|$ 0.0 / 0.1 &  \textbf{0.248} $|$ \underline{1.0} / 0.9 &  \textbf{0.749} $|$ \underline{1.0} / 0.4 &                       0.078 $|$ 0.0 / 0.7 \\
\midrule
Black-Box &  Max-Confidence &  \textbf{0.957} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.806} $|$ \underline{1.0} / \underline{1.0} &                      -0.024 $|$ 0.0 / 0.1 &  \textbf{0.741} $|$ \underline{1.0} / 0.6 &  \textbf{0.040} $|$ \underline{1.0} / 0.9 \\
\midrule
Isotonic Calibration &  Max-Confidence &              \textbf{0.956} $|$ \underline{1.0} / 0.7 &                                   0.796 $|$ 0.0 / 0.4 &                      -0.016 $|$ 0.0 / 0.1 &                       0.601 $|$ 0.0 / 0.3 &  \textbf{0.063} $|$ \underline{1.0} / 0.1 \\
\midrule
CP (Confidence) &          pvalue &                                   0.950 $|$ 0.0 / 0.3 &                                   0.740 $|$ 0.0 / 0.1 &                      -0.073 $|$ 0.0 / 0.1 &                       0.535 $|$ 0.0 / 0.3 &  \textbf{0.044} $|$ \underline{1.0} / 0.9 \\
&      confidence &                                   0.946 $|$ 0.0 / 0.1 &                                   0.709 $|$ 0.0 / 0.1 &                      -0.128 $|$ 0.0 / 0.0 &                       0.544 $|$ 0.0 / 0.1 &  \textbf{0.052} $|$ \underline{1.0} / 0.7 \\
 &     credibility &                                   0.946 $|$ 0.0 / 0.3 &                                   0.706 $|$ 0.0 / 0.1 &                      -0.100 $|$ 0.0 / 0.1 &                       0.519 $|$ 0.0 / 0.1 &  \textbf{0.053} $|$ \underline{1.0} / 0.7 \\
 &      efficiency &                                   0.940 $|$ 0.0 / 0.0 &                                   0.664 $|$ 0.0 / 0.0 &                      -0.097 $|$ 0.0 / 0.0 &                       0.389 $|$ 0.0 / 0.0 &                       0.191 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}

==> tables/intrinsic_binary_deep_ensemble.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                           error detection &                             ood detection &                           shift detection &                      perf drop prediction \\
\midrule

   Intrinsic &           Total &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.798} $|$ \underline{1.0} / 0.9 &                      -0.043 $|$ 0.0 / 0.1 &                       0.771 $|$ 0.0 / 0.4 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
     &       Aleatoric &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.796} $|$ \underline{1.0} / 0.7 &                      -0.136 $|$ 0.0 / 0.0 &                       0.746 $|$ 0.0 / 0.4 &                       0.092 $|$ 0.0 / 0.4 \\
     &       Epistemic &                                   0.947 $|$ 0.0 / 0.4 &                       0.748 $|$ 0.0 / 0.3 &  \textbf{0.289} $|$ \underline{1.0} / 0.9 &  \textbf{0.854} $|$ \underline{1.0} / 0.7 &                       0.092 $|$ 0.0 / 0.6 \\
\midrule
Black-Box &  Max-Confidence &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.798} $|$ \underline{1.0} / 0.9 &                      -0.043 $|$ 0.0 / 0.1 &                       0.771 $|$ 0.0 / 0.4 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
\midrule
    
    Isotonic Calibration & Max-Confidence &              \textbf{0.955} $|$ \underline{1.0} / 0.9 &                       0.792 $|$ 0.0 / 0.7 &                      -0.004 $|$ 0.0 / 0.1 &                       0.589 $|$ 0.0 / 0.3 &  \textbf{0.070} $|$ \underline{1.0} / 0.4 \\
\midrule

CP (confidence) &          pvalue &                                   0.947 $|$ 0.0 / 0.3 &                       0.725 $|$ 0.0 / 0.3 &                      -0.082 $|$ 0.0 / 0.3 &                       0.460 $|$ 0.0 / 0.0 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
                      
&     credibility &                                   0.944 $|$ 0.0 / 0.3 &                       0.698 $|$ 0.0 / 0.3 &                      -0.108 $|$ 0.0 / 0.3 &                       0.443 $|$ 0.0 / 0.1 &  \textbf{0.059} $|$ \underline{1.0} / 0.7 \\
 &      confidence &                                   0.944 $|$ 0.0 / 0.3 &                       0.695 $|$ 0.0 / 0.3 &                      -0.133 $|$ 0.0 / 0.1 &                       0.407 $|$ 0.0 / 0.0 &  \textbf{0.060} $|$ \underline{1.0} / 0.7 \\
 &      efficiency &                                   0.939 $|$ 0.0 / 0.0 &                       0.665 $|$ 0.0 / 0.0 &                      -0.099 $|$ 0.0 / 0.1 &                       0.328 $|$ 0.0 / 0.0 &                       0.204 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}




==> tables/intrinsic_multiclass.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                                         ood detection &                           shift detection &                      perf drop prediction \\
\midrule
 confidence conformal prediction &  non conformity &  \textbf{0.887} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.806} $|$ \underline{1.0} / \underline{1.0} &                                   0.044 $|$ 0.0 / 0.2 &              \textbf{0.981} $|$ 0.5 / 0.2 &  \textbf{0.097} $|$ \underline{1.0} / 0.8 \\
            isotonic calibration &  max confidence &  \textbf{0.887} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.805} $|$ \underline{1.0} / \underline{1.0} &                                   0.024 $|$ 0.0 / 0.0 &              \textbf{0.956} $|$ 0.5 / 0.2 &  \textbf{0.103} $|$ \underline{1.0} / 0.8 \\
            isotonic calibration &         entropy &              \textbf{0.886} $|$ 0.5 / \underline{1.0} &                                   0.800 $|$ 0.0 / 0.5 &                                  -0.039 $|$ 0.0 / 0.0 &              \textbf{0.962} $|$ 0.5 / 0.2 &                       0.108 $|$ 1.0 / 0.8 \\
                       intrinsic &           total &                                   0.886 $|$ 0.5 / 0.8 &                                   0.798 $|$ 0.0 / 0.2 &                                  -0.003 $|$ 0.0 / 0.2 &              \textbf{0.997} $|$ 0.5 / 0.2 &  \textbf{0.106} $|$ \underline{1.0} / 0.8 \\
                       intrinsic &       aleatoric &                                   0.886 $|$ 0.5 / 0.8 &                                   0.797 $|$ 0.0 / 0.2 &                                  -0.147 $|$ 0.0 / 0.2 &              \textbf{0.996} $|$ 0.5 / 0.2 &                       0.146 $|$ 0.5 / 0.5 \\
            isotonic calibration &          margin &                                   0.885 $|$ 0.0 / 0.8 &                                   0.799 $|$ 0.0 / 0.8 &                                   0.079 $|$ 0.0 / 0.0 &              \textbf{0.955} $|$ 0.5 / 0.2 &  \textbf{0.102} $|$ \underline{1.0} / 0.8 \\
 confidence conformal prediction &      confidence &                                   0.875 $|$ 0.0 / 0.0 &                                   0.747 $|$ 0.0 / 0.0 &                                   0.063 $|$ 0.0 / 0.0 &                       0.844 $|$ 0.0 / 0.2 &                       0.175 $|$ 0.0 / 0.0 \\
 confidence conformal prediction &      efficiency &                                   0.874 $|$ 0.0 / 0.0 &                                   0.710 $|$ 0.0 / 0.0 &                                  -0.136 $|$ 0.0 / 0.0 &                       0.628 $|$ 0.0 / 0.0 &                       0.222 $|$ 0.0 / 0.0 \\
 confidence conformal prediction &          pvalue &                                   0.872 $|$ 0.0 / 0.0 &                                   0.709 $|$ 0.0 / 0.0 &                                   0.022 $|$ 0.0 / 0.0 &                       0.745 $|$ 0.0 / 0.0 &                       0.120 $|$ 0.5 / 0.2 \\
 confidence conformal prediction &     credibility &                                   0.866 $|$ 0.0 / 0.0 &                                   0.685 $|$ 0.0 / 0.0 &                                  -0.008 $|$ 0.0 / 0.0 &                       0.749 $|$ 0.0 / 0.0 &                       0.115 $|$ 0.5 / 0.2 \\
                       intrinsic &       epistemic &                                   0.859 $|$ 0.0 / 0.0 &                                   0.665 $|$ 0.0 / 0.0 &  \textbf{0.438} $|$ \underline{1.0} / \underline{1.0} &  \textbf{1.000} $|$ \underline{1.0} / 0.5 &                       0.169 $|$ 0.0 / 0.5 \\
\bottomrule
\end{tabular}

==> tables/intrinsic_multiclass_cat_boost.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                                         ood detection &                           shift detection &                      perf drop prediction \\
\toprule

Intrinsic &           total &                                   0.882 $|$ 0.0 / 0.5 &                                   0.792 $|$ 0.0 / 0.2 &                                  -0.082 $|$ 0.0 / 0.2 &  \textbf{0.994} $|$ \underline{1.0} / 0.2 &  \textbf{0.120} $|$ \underline{1.0} / 0.5 \\

 &       aleatoric &                                   0.882 $|$ 0.0 / 0.5 &                                   0.792 $|$ 0.0 / 0.2 &                                  -0.083 $|$ 0.0 / 0.2 &  \textbf{0.997} $|$ \underline{1.0} / 0.2 &  \textbf{0.120} $|$ \underline{1.0} / 0.5 \\

 &       epistemic &                                   0.846 $|$ 0.0 / 0.0 &                                   0.611 $|$ 0.0 / 0.0 &  \textbf{0.373} $|$ \underline{1.0} / \underline{1.0} &  \textbf{1.000} $|$ \underline{1.0} / 0.5 &                       0.133 $|$ 0.0 / 0.8 \\

\midrule 


Isotonic Calibration &  max confidence &  \textbf{0.883} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.804} $|$ \underline{1.0} / \underline{1.0} &                                  -0.041 $|$ 0.0 / 0.0 &  \textbf{0.912} $|$ \underline{1.0} / 0.2 &  \textbf{0.120} $|$ \underline{1.0} / 0.5 \\

 &         entropy &                                   0.882 $|$ 0.0 / 0.8 &                                   0.798 $|$ 0.0 / 0.5 &                                  -0.120 $|$ 0.0 / 0.0 &  \textbf{0.925} $|$ \underline{1.0} / 0.2 &  \textbf{0.123} $|$ \underline{1.0} / 0.5 \\
 &          margin &                                   0.881 $|$ 0.0 / 0.8 &                                   0.797 $|$ 0.0 / 0.8 &                                   0.026 $|$ 0.0 / 0.0 &  \textbf{0.912} $|$ \underline{1.0} / 0.2 &  \textbf{0.118} $|$ \underline{1.0} / 0.5 \\
 \midrule
 CP (Confidence)  &          pvalue &                                   0.869 $|$ 0.0 / 0.0 &                                   0.711 $|$ 0.0 / 0.0 &                                  -0.039 $|$ 0.0 / 0.0 &                       0.741 $|$ 0.0 / 0.0 &  \textbf{0.122} $|$ \underline{1.0} / 0.5 \\

&      confidence &                                   0.869 $|$ 0.0 / 0.0 &                                   0.735 $|$ 0.0 / 0.0 &                                   0.049 $|$ 0.0 / 0.0 &                       0.792 $|$ 0.0 / 0.5 &                       0.179 $|$ 0.0 / 0.0 \\

 &     credibility &                                   0.863 $|$ 0.0 / 0.0 &                                   0.689 $|$ 0.0 / 0.0 &                                  -0.070 $|$ 0.0 / 0.0 &                       0.742 $|$ 0.0 / 0.0 &  \textbf{0.116} $|$ \underline{1.0} / 0.5 \\

  &      efficiency &                                   0.870 $|$ 0.0 / 0.0 &                                   0.700 $|$ 0.0 / 0.0 &                                  -0.201 $|$ 0.0 / 0.0 &                       0.483 $|$ 0.0 / 0.0 &                       0.243 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}


==> tables/intrinsic_multiclass_deep_ensemble.tex <==
\begin{tabular}{lllllll}
\toprule
                           model &           score &                                             retention &                                       error detection &                                         ood detection &                           shift detection &                      perf drop prediction \\
\toprule 

Intrinsic &           total &  \textbf{0.890} $|$ \underline{1.0} / \underline{1.0} &                                   0.803 $|$ 0.0 / 0.5 &                                   0.092 $|$ 0.0 / 0.2 &                       1.000 $|$ 0.0 / 0.2 &  \textbf{0.093} $|$ \underline{1.0} / 0.8 \\

 &       aleatoric &  \textbf{0.890} $|$ \underline{1.0} / \underline{1.0} &                                   0.801 $|$ 0.0 / 0.5 &                                  -0.212 $|$ 0.0 / 0.2 &                       0.998 $|$ 0.0 / 0.2 &                       0.172 $|$ 0.0 / 0.5 \\
 &       epistemic &                                   0.872 $|$ 0.0 / 0.2 &                                   0.718 $|$ 0.0 / 0.2 &  \textbf{0.504} $|$ \underline{1.0} / \underline{1.0} &  \textbf{1.000} $|$ \underline{1.0} / 0.2 &                       0.205 $|$ 0.0 / 0.5 \\
 \midrule

Black-Box &  Max-Confidence &  \textbf{0.891} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.807} $|$ \underline{1.0} / \underline{1.0} &                                   0.128 $|$ 0.0 / 0.2 &                       0.999 $|$ 0.0 / 0.2 &  \textbf{0.081} $|$ \underline{1.0} / 0.8 \\

\midrule

Isotonic Calibration &  max confidence &  \textbf{0.891} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.807} $|$ \underline{1.0} / \underline{1.0} &                                   0.101 $|$ 0.0 / 0.0 &                       1.000 $|$ 0.0 / 0.2 &  \textbf{0.086} $|$ \underline{1.0} / 0.8 \\
 &          margin &                                   0.889 $|$ 0.0 / 0.8 &                                   0.802 $|$ 0.0 / 0.8 &                                   0.146 $|$ 0.0 / 0.0 &                       1.000 $|$ 0.0 / 0.2 &  \textbf{0.086} $|$ \underline{1.0} / 0.8 \\
 &         entropy &  \textbf{0.890} $|$ \underline{1.0} / \underline{1.0} &                                   0.803 $|$ 0.0 / 0.5 &                                   0.050 $|$ 0.0 / 0.0 &                       1.000 $|$ 0.0 / 0.2 &  \textbf{0.093} $|$ \underline{1.0} / 0.8 \\
 \midrule 
 
CP (confidence) &      confidence &                                   0.881 $|$ 0.0 / 0.0 &                                   0.758 $|$ 0.0 / 0.0 &                                   0.067 $|$ 0.0 / 0.0 &                       0.910 $|$ 0.0 / 0.2 &                       0.170 $|$ 0.0 / 0.2 \\
 
 &          pvalue &                                   0.876 $|$ 0.0 / 0.0 &                                   0.706 $|$ 0.0 / 0.0 &                                   0.095 $|$ 0.0 / 0.0 &                       0.750 $|$ 0.0 / 0.0 &                       0.118 $|$ 0.0 / 0.2 \\

 &     credibility &                                   0.869 $|$ 0.0 / 0.0 &                                   0.681 $|$ 0.0 / 0.0 &                                   0.067 $|$ 0.0 / 0.0 &                       0.751 $|$ 0.0 / 0.0 &                       0.114 $|$ 0.0 / 0.2 \\
&      efficiency &                                   0.879 $|$ 0.0 / 0.0 &                                   0.721 $|$ 0.0 / 0.0 &                                  -0.059 $|$ 0.0 / 0.0 &                       0.788 $|$ 0.0 / 0.0 &                       0.201 $|$ 0.0 / 0.0 \\
\bottomrule
\end{tabular}

==> tables/summary_table_backup.tex <==
\begin{tabular}{lllllllll}
\toprule

            Base model             & UQ &           Score &                                             Retention &                                       Error Detection &                OoD Detection &             OoD Detection (AUC) &                           Shift Detection &                                  Perf. Drop Pred. \\
\toprule

Black-Box & None &  max confidence &  \textbf{0.948}
                       $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.790} $|$ \underline{1.0} / \underline{1.0} &          -0.008 $|$ 0.2 / 0.4 &           0.503 $|$ 0.2 / 0.6 &  \textbf{0.738} $|$ \underline{1.0} / 0.7 &  \textbf{0.100} $|$ \underline{1.0} / \underline{1.0} \\
\cmidrule{2-9}
         &   Isotonic Calibration &  max confidence &              \textbf{0.948} $|$ \underline{1.0} / 0.9 &                                   0.782 $|$ 0.2 / 0.9 &  \textbf{0.014} $|$ 0.8 / 0.4 &           0.496 $|$ 0.0 / 0.4 &                       0.604 $|$ 0.2 / 0.4 &                                   0.111 $|$ 0.2 / 0.1 \\
\cmidrule{2-9}
& CP (confidence) &          pvalue &                                   0.943 $|$ 0.0 / 0.4 &                                   0.735 $|$ 0.0 / 0.3 &          -0.040 $|$ 0.0 / 0.4 &  \textbf{0.508} $|$ 0.8 / 0.4 &                       0.595 $|$ 0.0 / 0.3 &                                   0.105 $|$ 1.0 / 0.6 \\
&  &     credibility &                                   0.937 $|$ 0.0 / 0.4 &                                   0.695 $|$ 0.0 / 0.3 &          -0.079 $|$ 0.0 / 0.4 &           0.505 $|$ 0.2 / 0.4 &                       0.538 $|$ 0.0 / 0.3 &                                   0.113 $|$ 0.2 / 0.4 \\
&  &      confidence &                                   0.937 $|$ 0.0 / 0.3 &                                   0.692 $|$ 0.0 / 0.3 &          -0.100 $|$ 0.0 / 0.0 &           0.497 $|$ 0.0 / 0.1 &                       0.480 $|$ 0.0 / 0.3 &                                   0.111 $|$ 0.5 / 0.6 \\
&  &      efficiency &                                   0.932 $|$ 0.0 / 0.0 &                                   0.657 $|$ 0.0 / 0.0 &          -0.067 $|$ 0.0 / 0.4 &           0.499 $|$ 0.2 / 0.3 &                       0.377 $|$ 0.0 / 0.1 &                                   0.219 $|$ 0.0 / 0.1 \\
\cmidrule{2-9}

& CP (Anomaly score) &  non conformity &                       0.922 $|$ 0.0 / 0.0 &                                   0.626 $|$ 0.0 / 0.0 &  \textbf{0.798} $|$ \underline{1.0} / 0.7 &                       0.638 $|$ 0.8 / 0.4 &  \textbf{0.915} $|$ \underline{1.0} / 0.6 &                       0.178 $|$ 0.0 / 0.4 \\

&  &          pvalue &                       0.920 $|$ 0.0 / 0.0 &                                   0.604 $|$ 0.0 / 0.0 &                       0.777 $|$ 0.2 / 0.1 &  \textbf{0.641} $|$ \underline{1.0} / 0.6 &                       0.852 $|$ 0.0 / 0.3 &                       0.178 $|$ 0.0 / 0.6 \\
&  &      confidence &                       0.919 $|$ 0.0 / 0.0 &                                   0.546 $|$ 0.0 / 0.0 &                      -0.814 $|$ 0.0 / 0.0 &                       0.415 $|$ 0.0 / 0.1 &                       0.864 $|$ 0.2 / 0.4 &                       0.154 $|$ 0.0 / 0.0 \\
&  &     credibility &                       0.917 $|$ 0.0 / 0.0 &                                   0.573 $|$ 0.0 / 0.0 &                       0.789 $|$ 0.5 / 0.6 &              \textbf{0.640} $|$ 0.8 / 0.6 &                       0.849 $|$ 0.0 / 0.3 &                       0.180 $|$ 0.0 / 0.6 \\

&  &      efficiency &                       0.918 $|$ 0.0 / 0.0 &                                   0.553 $|$ 0.0 / 0.0 &                       0.108 $|$ 0.0 / 0.0 &                       0.533 $|$ 0.0 / 0.0 &                       0.337 $|$ 0.0 / 0.0 &                       0.147 $|$ 0.0 / 0.1 \\
\bottomrule
\toprule

Deep Ensemble & Intrinsic &           Total &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.798} $|$ \underline{1.0} / 0.9 &                      -0.043 $|$ 0.0 / 0.1 &   &                    0.771 $|$ 0.0 / 0.4 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
\citep{lakshminarayanan2017simple} &     &       Aleatoric &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.796} $|$ \underline{1.0} / 0.7 &                      -0.136 $|$ 0.0 / 0.0 &  &                       0.746 $|$ 0.0 / 0.4 &                       0.092 $|$ 0.0 / 0.4 \\
&     &       Epistemic &                                   0.947 $|$ 0.0 / 0.4 &                       0.748 $|$ 0.0 / 0.3 &  \textbf{0.289} $|$ \underline{1.0} / 0.9 & &  \textbf{0.854} $|$ \underline{1.0} / 0.7  &                      0.092 $|$ 0.0 / 0.6 \\
\cmidrule{2-9}
& None &  Max-Confidence &  \textbf{0.955} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.798} $|$ \underline{1.0} / 0.9 &                      -0.043 $|$ 0.0 / 0.1 & &                      0.771 $|$ 0.0 / 0.4 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
\cmidrule{2-9}

&    Isotonic Calibration & Max-Confidence & \textbf{0.955} $|$ \underline{1.0} / 0.9 &                       0.792 $|$ 0.0 / 0.7 &                      -0.004 $|$ 0.0 / 0.1 &     &                   0.589 $|$ 0.0 / 0.3 &  \textbf{0.070} $|$ \underline{1.0} / 0.4 \\
\cmidrule{2-9}

 & CP (confidence) &          pvalue &                                   0.947 $|$ 0.0 / 0.3 &                       0.725 $|$ 0.0 / 0.3 &                      -0.082 $|$ 0.0 / 0.3 &  &                       0.460 $|$ 0.0 / 0.0 &  \textbf{0.056} $|$ \underline{1.0} / 0.7 \\
                      
& &     credibility &                                   0.944 $|$ 0.0 / 0.3 &                       0.698 $|$ 0.0 / 0.3 &                      -0.108 $|$ 0.0 / 0.3 &   &                    0.443 $|$ 0.0 / 0.1 &  \textbf{0.059} $|$ \underline{1.0} / 0.7 \\
&  &      confidence &                                   0.944 $|$ 0.0 / 0.3 &                       0.695 $|$ 0.0 / 0.3 &                      -0.133 $|$ 0.0 / 0.1 &   &                    0.407 $|$ 0.0 / 0.0 &  \textbf{0.060} $|$ \underline{1.0} / 0.7 \\
& &      efficiency &                                   0.939 $|$ 0.0 / 0.0 &                       0.665 $|$ 0.0 / 0.0 &                      -0.099 $|$ 0.0 / 0.1 &  &                     0.328 $|$ 0.0 / 0.0 &                       0.204 $|$ 0.0 / 0.0 \\
 \bottomrule
 \toprule
 
Cat Boost & Intrinsic &           total &              \textbf{0.957} $|$ \underline{1.0} / 0.9 &              \textbf{0.806} $|$ \underline{1.0} / 0.9 &                      -0.012 $|$ 0.0 / 0.1 &  & \textbf{0.752} $|$ \underline{1.0} / 0.4 &  \textbf{0.042} $|$ \underline{1.0} / 0.9 \\
\citep{Malinin2021} &  &       aleatoric &              \textbf{0.957} $|$ \underline{1.0} / 0.9 &              \textbf{0.806} $|$ \underline{1.0} / 0.9 &                      -0.013 $|$ 0.0 / 0.1 & &  \textbf{0.768} $|$ \underline{1.0} / 0.6 &  \textbf{0.042} $|$ \underline{1.0} / 0.9 \\
 & &       epistemic &                                   0.939 $|$ 0.0 / 0.1 &                                   0.676 $|$ 0.0 / 0.1 &  \textbf{0.248} $|$ \underline{1.0} / 0.9 & &  \textbf{0.749} $|$ \underline{1.0} / 0.4 &                       0.078 $|$ 0.0 / 0.7 \\
\cmidrule{2-9}
& None &  Max-Confidence &  \textbf{0.957} $|$ \underline{1.0} / \underline{1.0} &  \textbf{0.806} $|$ \underline{1.0} / \underline{1.0} &                      -0.024 $|$ 0.0 / 0.1 & &  \textbf{0.741} $|$ \underline{1.0} / 0.6 &  \textbf{0.040} $|$ \underline{1.0} / 0.9 \\
\cmidrule{2-9}
& Isotonic Calibration &  Max-Confidence &              \textbf{0.956} $|$ \underline{1.0} / 0.7 &                                   0.796 $|$ 0.0 / 0.4 &                      -0.016 $|$ 0.0 / 0.1 & &                       0.601 $|$ 0.0 / 0.3 &  \textbf{0.063} $|$ \underline{1.0} / 0.1 \\
\cmidrule{2-9}
& CP (Confidence) &          pvalue &                                   0.950 $|$ 0.0 / 0.3 &                                   0.740 $|$ 0.0 / 0.1 &                      -0.073 $|$ 0.0 / 0.1 &  &                     0.535 $|$ 0.0 / 0.3 &  \textbf{0.044} $|$ \underline{1.0} / 0.9 \\
& &      confidence &                                   0.946 $|$ 0.0 / 0.1 &                                   0.709 $|$ 0.0 / 0.1 &                      -0.128 $|$ 0.0 / 0.0 &  &                     0.544 $|$ 0.0 / 0.1 &  \textbf{0.052} $|$ \underline{1.0} / 0.7 \\
&  &     credibility &                                   0.946 $|$ 0.0 / 0.3 &                                   0.706 $|$ 0.0 / 0.1 &                      -0.100 $|$ 0.0 / 0.1 &  &                      0.519 $|$ 0.0 / 0.1 &  \textbf{0.053} $|$ \underline{1.0} / 0.7 \\
&  &      efficiency &                                   0.940 $|$ 0.0 / 0.0 &                                   0.664 $|$ 0.0 / 0.0 &                      -0.097 $|$ 0.0 / 0.0 &  &                     0.389 $|$ 0.0 / 0.0 &                       0.191 $|$ 0.0 / 0.0 \\
\bottomrule
\toprule 



\end{tabular}
